Correlations of the elements of the neutrino mass matrix

Assuming Majorana nature of neutrinos, we re-investigate, in the light of the recent measurement of the reactor mixing angle, the allowed ranges for the absolute values of the elements of the neutrino mass matrix in the basis where the charged-lepton mass matrix is diagonal. Apart from the derivation of upper and lower bounds on the values of the matrix elements, we also study their correlations. Moreover, we analyse the sensitivity of bounds and correlations to the global fit results of the neutrino oscillation parameters which are available in the literature.

==> PaxHeaders.7387/correlations-arXiv2.tex <==
30 mtime=1355995979.065495682
30 atime=1355995987.997495774
30 ctime=1355995979.125535232

